Photoproduction of two charged pions off protons in the resonance region

Photoproduction of charged pions pairs off protons is studied within the invariant masses of the final state hadrons from 1.6 to 2.4 GeV at the Thomas Jefferson National Accelerator Facility with the CLAS detector. The data are included in the Bonn-Gatchina coupled-channel analysis and provide the information necessary to determine the branching fractions for most known nucleon and Delta resonances. Branching ratios are obtained here from an event based likelihood fit.

==> main-authors.tex <==
\newcommand*{\ANL}{Argonne National Laboratory, Argonne, Illinois 60439, United States of America}
\newcommand*{\ANLindex}{1}
\affiliation{\ANL}
\newcommand*{\ASU}{Arizona State University, Tempe, Arizona 85287, United States of America}
\newcommand*{\ASUindex}{2}
\affiliation{\ASU}
\newcommand*{\CSUDH}{California State University, Dominguez Hills, Carson, California 90747, United States of America}
\newcommand*{\CSUDHindex}{3}
\affiliation{\CSUDH}
\newcommand*{\CANISIUS}{Canisius College, Buffalo, New York 14208, United States of America}
\newcommand*{\CANISIUSindex}{4}
\affiliation{\CANISIUS}
\newcommand*{\CMU}{Carnegie Mellon University, Pittsburgh, Pennsylvania 15213, United States of America}
\newcommand*{\CMUindex}{5}
\affiliation{\CMU}
\newcommand*{\CUA}{The Catholic University of America, Washington, District of Columbia 20064, United States of America}
\newcommand*{\CUAindex}{6}
\affiliation{\CUA}
\newcommand*{\SACLAY}{IRFU, CEA, Universit\`{e} Paris-Saclay, F-91191 Gif-sur-Yvette, France}
\newcommand*{\SACLAYindex}{7}
\affiliation{\SACLAY}
\newcommand*{\CNU}{Christopher Newport University, Newport News, Virginia 23606, United States of America}
\newcommand*{\CNUindex}{8}
\affiliation{\CNU}
\newcommand*{\UCONN}{University of Connecticut, Storrs, Connecticut 06269, United States of America}
\newcommand*{\UCONNindex}{9}
\affiliation{\UCONN}
\newcommand*{\DUQUESNE}{Duquesne University, Pittsburgh, Pennsylvania 15282, United States of America }
\newcommand*{\DUQUESNEindex}{10}
\affiliation{\DUQUESNE}
\newcommand*{\FU}{Fairfield University, Fairfield, Connecticut 06824, United States of America}
\newcommand*{\FUindex}{11}
\affiliation{\FU}
\newcommand*{\FERRARAU}{Universit\`a di Ferrara, 44121 Ferrara, Italy}
\newcommand*{\FERRARAUindex}{12}
\affiliation{\FERRARAU}
\newcommand*{\FIU}{Florida International University, Miami, Florida 33199, United States of America}
\newcommand*{\FIUindex}{13}
\affiliation{\FIU}
\newcommand*{\FSU}{Florida State University, Tallahassee, Florida 32306, United States of America}
\newcommand*{\FSUindex}{14}
\affiliation{\FSU}
\newcommand*{\GWUI}{The George Washington University, Washington, District of Columbia 20052, United States of America}
\newcommand*{\GWUIindex}{15}
\affiliation{\GWUI}
\newcommand*{\GSIFFN}{GSI Helmholtzzentrum fur Schwerionenforschung GmbH, D-64291 Darmstadt, Germany}
\newcommand*{\GSIFFNindex}{16}
\affiliation{\GSIFFN}
\newcommand*{\INFNFE}{INFN, Sezione di Ferrara, 44100 Ferrara, Italy}
\newcommand*{\INFNFEindex}{17}
\affiliation{\INFNFE}
\newcommand*{\INFNGE}{INFN, Sezione di Genova, 16146 Genova, Italy}
\newcommand*{\INFNGEindex}{18}
\affiliation{\INFNGE}
\newcommand*{\INFNRO}{INFN, Sezione di Roma Tor Vergata, 00133 Rome, Italy}
\newcommand*{\INFNROindex}{19}
\affiliation{\INFNRO}
\newcommand*{\INFNTUR}{INFN, Sezione di Torino, 10125 Torino, Italy}
\newcommand*{\INFNTURindex}{20}
\affiliation{\INFNTUR}
\newcommand*{\INFNPAV}{INFN, Sezione di Pavia, 27100 Pavia, Italy}
\newcommand*{\INFNPAVindex}{21}
\affiliation{\INFNPAV}
\newcommand*{\IFKMA}{Institut f\"ur Kernphysik, Johannes Gutenberg University of Mainz, D-55099 Mainz, Germany}
\newcommand*{\IFKMAindex}{22}
\affiliation{\IFKMA}
\newcommand*{\KNU}{Kyungpook National University, Daegu 41566, South Korea}
\newcommand*{\KNUindex}{23}
\affiliation{\KNU}
\newcommand*{\LAMAR}{Lamar University, Beaumont, Texas 77710, United States of America}
\newcommand*{\LAMARindex}{24}
\affiliation{\LAMAR}
\newcommand*{\MIT}{Massachusetts Institute of Technology, Cambridge, Massachusetts  02139, United States of America}
\newcommand*{\MITindex}{25}
\affiliation{\MIT}
\newcommand*{\MISS}{Mississippi State University, Mississippi State, Mississippi 39762, United States of America}
\newcommand*{\MISSindex}{26}
\affiliation{\MISS}
\newcommand*{\ITEP}{National Research Centre Kurchatov Institute - ITEP, Moscow, 117259, Russia}
\newcommand*{\ITEPindex}{27}
\affiliation{\ITEP}
\newcommand*{\NMSU}{New Mexico State University, Las Cruces, New Mexico 88003, United States of America}
\newcommand*{\NMSUindex}{28}
\affiliation{\NMSU}
\newcommand*{\NSU}{Norfolk State University, Norfolk, Virginia 23504, United States of America}
\newcommand*{\NSUindex}{29}
\affiliation{\NSU}
\newcommand*{\NRC}{NRC Kurchatov Institute, PNPI, Gatchina 188300, Russia}
\newcommand*{\NRCindex}{30}
\affiliation{\NRC}
\newcommand*{\OHIOU}{Ohio University, Athens, Ohio 45701, United States of America}
\newcommand*{\OHIOUindex}{31}
\affiliation{\OHIOU}
\newcommand*{\ODU}{Old Dominion University, Norfolk, Virginia 23529, United States of America}
\newcommand*{\ODUindex}{32}
\affiliation{\ODU}
\newcommand*{\JLUGiessen}{II Physikalisches Institut, Justus Liebig University Giessen, 35392 Giessen, Germany}
\newcommand*{\JLUGiessenindex}{33}
\affiliation{\JLUGiessen}
\newcommand*{\MSU}{Skobeltsyn Institute of Nuclear Physics, Lomonosov Moscow State University, 119234 Moscow, Russia}
\newcommand*{\MSUindex}{34}
\affiliation{\MSU}
\newcommand*{\TEMPLE}{Temple University,  Philadelphia, Pennsylvania 19122, United States of America }
\newcommand*{\TEMPLEindex}{35}
\affiliation{\TEMPLE}
\newcommand*{\ORSAY}{Universit\`{e} Paris-Saclay, CNRS/IN2P3, IJCLab, 91405 Orsay, France}
\newcommand*{\ORSAYindex}{37}
\affiliation{\ORSAY}
\newcommand*{\UNH}{University of New Hampshire, Durham, New Hampshire 03824, United States of America}
\newcommand*{\UNHindex}{38}
\affiliation{\UNH}
\newcommand*{\URICH}{University of Richmond, Richmond, Virginia 23173, United States of America}
\newcommand*{\URICHindex}{39}
\affiliation{\URICH}
\newcommand*{\ROMAII}{Universit\`a di Roma Tor Vergata, 00133 Rome Italy}
\newcommand*{\ROMAIIindex}{40}
\affiliation{\ROMAII}
\newcommand*{\SCAROLINA}{University of South Carolina, Columbia, South Carolina 29208, United States of America}
\newcommand*{\SCAROLINAindex}{41}
\affiliation{\SCAROLINA}
\newcommand*{\UTFSM}{Universidad T\`{e}cnica Federico Santa Mar\'{i}a, Casilla 110-V Valpara\`{i}so, Chile}
\newcommand*{\UTFSMindex}{42}
\affiliation{\UTFSM}
\newcommand*{\BRESCIA}{Universit\`{a} degli Studi di Brescia, 25123 Brescia, Italy}
\newcommand*{\BRESCIAindex}{43}
\affiliation{\BRESCIA}
\newcommand*{\UCR}{University of California Riverside, Riverside, California 92521, United States of America}
\newcommand*{\UCRindex}{44}
\affiliation{\UCR}
\newcommand*{\GLASGOW}{University of Glasgow, Glasgow G12 8QQ, United Kingdom}
\newcommand*{\GLASGOWindex}{45}
\affiliation{\GLASGOW}
\newcommand*{\YORK}{University of York, York YO10 5DD, United Kingdom}
\newcommand*{\YORKindex}{46}
\affiliation{\YORK}
\newcommand*{\VT}{Virginia Polytechnic Institute and State University, Blacksburg, Virginia 24061, United States of America}
\newcommand*{\VTindex}{47}
\affiliation{\VT}
\newcommand*{\VIRGINIA}{University of Virginia, Charlottesville, Virginia 22901, United States of America}
\newcommand*{\VIRGINIAindex}{48}
\affiliation{\VIRGINIA}
\newcommand*{\WM}{College of William and Mary, Williamsburg, Virginia 23187, United States of America}
\newcommand*{\WMindex}{49}
\affiliation{\WM}
\newcommand*{\YEREVAN}{Yerevan Physics Institute, 375036 Yerevan, Armenia}
\newcommand*{\YEREVANindex}{50}
\affiliation{\YEREVAN}
\newcommand*{\NOWJLAB}{Thomas Jefferson National Accelerator Facility, Newport News, Virginia 23606, United States of America}
\newcommand*{\NOWVIRGINIA}{University of Virginia, Charlottesville, Virginia 22901, United States of America}
\newcommand*{\NOWMERYLAND}{Montgomery College, Germantown, Maryland 20876, United States of America}
 %%%%%%%%%%%%%%% END OF Latex Macros for institute addresses  %%%%%%%%%%%%%%%%%%%%%%%%%





\author {Z.~Akbar}
\affiliation{\VIRGINIA}
\author {M.J.~Amaryan}
\affiliation{\ODU}
\author{\mbox{G.~Angelini}}
\affiliation{\GWUI}
\author {W.R.~Armstrong}
\affiliation{\ANL}
\author {H.~Atac}
\affiliation{\TEMPLE}
\author {L.~Baashen}
\affiliation{\FIU}
\author {N.A.~Baltzell}
\affiliation{\JLAB}
\affiliation{\SCAROLINA}
\author {L.~Barion}
\affiliation{\INFNFE}
\author{\mbox{M.~Bashkanov}}
\affiliation{\YORK}
\author {M.~Battaglieri}
\affiliation{\INFNGE}
\author {I.~Bedlinskiy}
\affiliation{\ITEP}
\author {B.~Benkel}
\affiliation{\UTFSM}
\author {F.~Benmokhtar}
\affiliation{\DUQUESNE}
\author{\mbox{N.~Benmouna}}
\altaffiliation[Current address:]{\NOWMERYLAND}
% \altaffiliation{Current address:  Montgomery College, Germantown, Maryland 20876, United States of America}
\affiliation{\GWUI}
\author {A.~Bianconi}
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {A.S.~Biselli}
\affiliation{\FU}
\author {W.A.~Booth}
\affiliation{\YORK}
\author {F.~Boss\`u}
\affiliation{\SACLAY}
\author {S.~Boiarinov}
\affiliation{\JLAB}
\author {K.T.~Brinkmann}
\affiliation{\JLUGiessen}
\author{\mbox{W.~J.~Briscoe}}
\affiliation{\GWUI}
\author{\mbox{J.~Brock}}
\affiliation{\JLAB}
\author {D.~Bulumulla}
\affiliation{\ODU}
\author {T.~Cao}
\affiliation{\JLAB}
\author{\mbox{C.~Carlin}}
\affiliation{\JLAB}
\author {D.~S.~Carman}
\affiliation{\JLAB}
\author {J.C.~Carvajal}
\affiliation{\FIU}
\author {P.~Chatagnon}
\affiliation{\JLAB}
\author {V.~Chesnokov}
\affiliation{\MSU}
\author {T.~Chetry}
\affiliation{\FIU}
\author {G.~Ciullo}
\affiliation{\INFNFE}
\affiliation{\FERRARAU}
\author {G.~Clash}
\affiliation{\YORK}
\author {P.L.~Cole}
\affiliation{\LAMAR}
\author {M.~Contalbrigo}
\affiliation{\INFNFE}
\author{\mbox{O.~Cortes~Becerra}}
\affiliation{\GWUI}
\author {G.~Costantini}
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {A.~D'Angelo}
\affiliation{\INFNRO}
\affiliation{\ROMAII}
\author {N.~Dashyan}
\affiliation{\YEREVAN}
\author {R.~De~Vita}
\affiliation{\INFNGE}
\affiliation{\JLAB}
\author {M.~Defurne}
\affiliation{\SACLAY}
\author {A.~Deur}
\affiliation{\JLAB}
\author {S.~Diehl}
\affiliation{\JLUGiessen}
\affiliation{\UCONN}
\author {C.~Djalali}
\affiliation{\OHIOU}
\affiliation{\SCAROLINA}
\author {M.~Dugger}
\affiliation{\ASU}
\author {R.~Dupre}
\affiliation{\ORSAY}
\author {H.~Egiyan}
\affiliation{\JLAB}
\affiliation{\UNH}
\author {A.~El~Alaoui}
\affiliation{\UTFSM}
\author {L.~El~Fassi}
\affiliation{\MISS}
\affiliation{\ANL}
\author {L.~Elouadrhiri}
\affiliation{\JLAB}
\author {P.~Eugenio}
\affiliation{\FSU}
\author{\mbox{S.~Fegan}}
 \affiliation{\YORK}
\author {A.~Filippi}
\affiliation{\INFNTUR}
\author {C.~Fogler}
\affiliation{\ODU}
\author {G.~Gavalian}
\affiliation{\JLAB}
\affiliation{\ODU}
\author {G.~P.~Gilfoyle}
\affiliation{\URICH}
\author {A.~A.~Golubenko}
\affiliation{\MSU}
\author{G.~Gosta}
\affiliation{\INFNPAV}
\author {R.~W.~Gothe}
\affiliation{\SCAROLINA}
\author {K.~A.~Griffioen}
\affiliation{\WM}
\author {K.~Hafidi}
\affiliation{\ANL}
\author {H.~Hakobyan}
\affiliation{\UTFSM}
\affiliation{\YEREVAN}
\author {M.~Hattawy}
\affiliation{\ODU}
\author {F.~Hauenstein}
\affiliation{\JLAB}
\author {T.B.~Hayward}
\affiliation{\UCONN}
\author {D.~Heddle}
\affiliation{\CNU}
\affiliation{\JLAB}
\author {A.~Hobart}
\affiliation{\ORSAY}
\author {M.~Holtrop}
\affiliation{\UNH}
\author {Y.~Ilieva}
\affiliation{\SCAROLINA}
\affiliation{\GWUI}
\author{\mbox{I.~Illari}}
\affiliation{\GWUI}
\author {D.G.~Ireland}
\affiliation{\GLASGOW}
\author {E.L.~Isupov}
\affiliation{\MSU}
\author{\mbox{H.~Iwamoto}}
\affiliation{\GWUI}
\author {D.~Jenkins}
\affiliation{\VT}
\author {H.~S.~Jo}
\affiliation{\KNU}
\author {R.~Johnston}
\affiliation{\MIT}
\author {K.~Joo}
\affiliation{\UCONN}
\author {S.~Joosten}
\affiliation{\ANL}
\author {T.~Kageya}
\affiliation{\JLAB}
\author{\mbox{V.L.~Kashevarov}}
\affiliation{\IFKMA}
\author{\mbox{C.~D.~Keith}}
\affiliation{\JLAB}
\author {D.~Keller}
\affiliation{\VIRGINIA}
\affiliation{\OHIOU}
\author {A.~Khanal}
\affiliation{\FIU}
\author {A.~Kim}
\affiliation{\UCONN}
\author{\mbox{C.~W.~Kim}}
\affiliation{\GWUI}
\author {W.~Kim}
\affiliation{\KNU}
\author {F.~J.~Klein}
\affiliation{\CUA}
\author {V.~Klimenko}
\affiliation{\UCONN}
\author {A.~Kripko}
\affiliation{\JLUGiessen}
\author {V.~Kubarovsky}
\affiliation{\JLAB}
\author {L.~Lanza}
\affiliation{\INFNRO}
\affiliation{\ROMAII}
\author {M.~Leali}
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {S.~Lee}
\affiliation{\ANL}
\author {X.~Li}
\affiliation{\MIT}
\author {K.~Livingston}
\affiliation{\GLASGOW}
\author {I.J.D.~MacGregor}
\affiliation{\GLASGOW}
\author {D.~Marchand}
\affiliation{\ORSAY}
\author {V.~Mascagna}
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {B.~McKinnon}
\affiliation{\GLASGOW}
\author {S.~Migliorati}
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {R.G.~Milner}
\affiliation{\MIT}
\author {T.~Mineeva}
\affiliation{\UTFSM}
\author {C.~Munoz~Camacho}
\affiliation{\ORSAY}
\author {P.~Nadel-Turonski}
\affiliation{\JLAB}
\affiliation{\CUA}
\author {K.~Neupane}
\affiliation{\SCAROLINA}
\author {S.~Niccolai}
\affiliation{\ORSAY}
\author {M.~Osipenko}
\affiliation{\INFNGE}
\author {A.I.~Ostrovidov}
\affiliation{\FSU}
\author {P.~Pandey}
\affiliation{\ODU}
\author {M.~Paolone}
\affiliation{\NMSU}
\author {L.L.~Pappalardo}
\affiliation{\INFNFE}
\affiliation{\FERRARAU}
\author {R.~Paremuzyan}
\affiliation{\JLAB}
\author {E.~Pasyuk}
\affiliation{\JLAB}
\author {S.J.~Paul}
\affiliation{\UCR}
\author {N.~Pilleux}
\affiliation{\ORSAY}
\author {M.~Pokhrel}
\affiliation{\ODU}
\author {J.~Poudel}
\altaffiliation[Current address:]{\NOWJLAB}
\affiliation{\ODU}
\author {J.W.~Price}
\affiliation{\CSUDH}
\author {Y.~Prok}
\affiliation{\ODU}
\affiliation{\VIRGINIA}
\author {A.~Radic}
\affiliation{\UTFSM}
\author {N.~Ramasubramanian}
\affiliation{\SACLAY}
\author{\mbox{S.~Ratliff}}
\affiliation{\GWUI}
\author {T.~Reed}
\affiliation{\FIU}
\author {J.~Richards}
\affiliation{\UCONN}
\author {M.~Ripani}
\affiliation{\INFNGE}
\author {B.G.~Ritchie}
\affiliation{\ASU}
\author {J.~Ritman}
\affiliation{\GSIFFN}
\author {G.~Rosner}
\affiliation{\GLASGOW}
\author {C.~Salgado}
\affiliation{\NSU}
\author {S.~Schadmand}
\affiliation{\GSIFFN}
\author{\mbox{A.~Schmidt}}
\affiliation{\GWUI}
\author{\mbox{D.~Schott}}
\altaffiliation{Current address: University of Nebraska,
        Omaha, Nebraska 68198, United States of America}
\affiliation{\GWUI}
\author {R.A.~Schumacher}
\affiliation{\CMU}
\author {M.B.C~Scott}
\affiliation{\ANL}
\author{\mbox{M.L.~Seely}}
\affiliation{\JLAB}
\author{\mbox{E.M.~Seroka}}
\affiliation{\GWUI}
\author {E.V.~Shirokov}
\affiliation{\MSU}
\author {U.~Shrestha}
\affiliation{\UCONN}
\author {D.~Sokhan}
\affiliation{\SACLAY}
\affiliation{\GLASGOW}
\author {N.~Sparveris}
\affiliation{\TEMPLE}
\author {M.~Spreafico}
\affiliation{\INFNGE}
\author{\mbox{I.I.~Strakovsky}}
\affiliation{\GWUI}
\author {S.~Strauch}
\affiliation{\SCAROLINA}
\author {J.~Tan}
\affiliation{\KNU}
\author {R.~Tyson}
\affiliation{\GLASGOW}
\author {M.~Ungaro}
\affiliation{\JLAB}
\affiliation{\UCONN}
\author {S.~Vallarino}
\affiliation{\INFNFE}
\author {L.~Venturelli}
\affiliation{\BRESCIA}
\affiliation{\INFNPAV}
\author {H.~Voskanyan}
\affiliation{\YEREVAN}
\author{E.~Voutier}
\affiliation{\ORSAY}
\author{\mbox{D.~P.~Watts}}
\affiliation{\YORK}
\author {X.~Wei}
\affiliation{\JLAB}
\author {R.~Williams}
\affiliation{\YORK}
\author {R.~Wishart}
\affiliation{\GLASGOW}
\author {M.~H.~Wood}
\affiliation{\CANISIUS}
\affiliation{\SCAROLINA}
\author{\mbox{R.L.~Workman}}
\affiliation{\GWUI}
\author{M.~Yurov}
\affiliation{\MISS}
\author{\mbox{N.~Zachariou}}
\affiliation{\YORK}
\author {J.~Zhang}
\altaffiliation[Current address:]{\NOWVIRGINIA}
\affiliation{\ODU}
\author {M.~Zurek}
\affiliation{\ANL}
